Differential Operator Representation of sl (2, R) as Modules over Univariate and Bivariate Hermite Polynomials

This paper presents the connections between univariate and bivariate Hermite polynomials and associated differential equations with specific representations of Lie algebra sl(2,R) whose Cartan sub-algebras coincide the associated differential operators of these differential equations . Applying the Baker-Campbell-Hausdorff formula to generators of these algebras, results in new relation for one-variable and Bivariate Hermite polynomials. A general form of sl(2,R) representation by differential operators and arbitrary polynomial basis such as Laguerre and Legendre polynomials is introduced.

==> amiri.tex <==
\text{This paper presents the connections between one-variable and bivariate Hermite differential equations and associated Hermite polynomials with spwcific representations of sl(2,R) Lie algebra whose Cartan sub-algebras coincides with the differential operators of these differential equations . Applying the Baker-Campbell-Hausdorff formula to these algebras, results in new relations and generating functions in one-variable and Bivariate Hermite polynomials. A general form of sl(2,R) representation for other orthogonal polynomials such as Laguerre polynomials is introduced.}
\textbf{1. Introduction} 
\text{Hermite polynomials are among the most applicable special functions. These polynomials arise in 
diverse fields of probability, physics, numerical analysis, and signal processing. As an example, in quantum mechanics, eigenfunction solutions to quantum harmonic oscillators are described in terms of Hermite polynomials. Bivariate Hermite polynomials are useful in algebraic geometry and two-dimensional quantum harmonic oscillators [3,4,5]. Concerning the field of applications, Hermite polynomials in one variable are divided into probabilist and physicist versions. In the present paper, we focus on one and two-dimensional probabilist Hermite polynomials. We prove the symmetries of associated differential equations are compatible with sl(2,R) algebra. By introducing isomorphic Lie algebras whose Cartan sub-algebras are the Hermite differential operators, applying the Baker-Campbell-Hausdorff formula yields new relations for one variable and bivariate Hermite polynomials. Without exception, all known generating functions for Hermite polynomials contain a factorial term in the denominator. We introduce a new generating function without a factorial denominator.}
\text{Hermite polynomials are among the most applicable special functions. These polynomials arise in 
diverse fields of probability, physics, numerical analysis, and signal processing. As an example, in quantum mechanics, eigenfunction solutions to quantum harmonic oscillators are described in terms of Hermite polynomials. Bivariate Hermite polynomials are useful in algebraic geometry and two-dimensional quantum harmonic oscillators [3,4,5]. Concerning the field of applications, Hermite polynomials in one variable are divided into probabilist and physicist versions. In the present paper, we focus on one and two-dimensional probabilist Hermite polynomials. We prove the symmetries of associated differential equations are compatible with sl(2,R) algebra. By introducing isomorphic Lie algebras whose Cartan sub-algebras are the Hermite differential operators, applying the Baker-Campbell-Hausdorff formula yields new relations for one variable and bivariate Hermite polynomials. Without exception, all known generating functions for Hermite polynomials contain a factorial term in the denominator. We introduce a new generating function without a factorial denominator.
H_{n}^e\left( x \right)=e^{-\frac{D^{2}}{2}}x^{n}
